Inflation, Universality and Attractors

In this PhD thesis, we investigate generic features of inflation which are strictly related to fundamental aspects of UV-physics scenarios, such as string theory or supergravity. After a short introduction to standard and inflationary cosmology, we present our research findings. On the one hand, we show that focusing on universality properties of inflation can yield surprisingly stringent bounds on its dynamics. This approach allows us to identify the regime where the inflationary field range is uniquely determined by both the tensor-to-scalar ratio and the spectral index. Then, we derive a novel field-range bound, which is two orders of magnitude stronger than the original one derived by Lyth. On the other hand, we discuss the embedding of inflation in supergravity and prove that non-trivial hyperbolic K\"ahler geometries induce an attractor for the inflationary observables: the spectral tilt tends automatically to the center of the Planck dome whereas the amount of primordial gravitational waves is directly controlled by curvature of the internal manifold. We identify the origin of this attractor mechanism in the so-called $\alpha$-scale supergravity model. Finally, we show how the inclusion of a nilpotent sector, allowing for a unified description of inflation and dark energy, implies an enhancement of the attractor nature of the theory. The main results of this thesis have been already published elsewhere. However, here we pay special attention to present them in a comprehensive way and provide the reader with the necessary background.

==> chapters/Attractors.tex <==
%\renewcommand{\chapterheadstartvskip}{\vspace*{-3.5\baselineskip}}

\chapter{Cosmological $\alpha$-Attractors}
\label{chapter:Attractors}

\section{Introduction}



==> preamble/equations.tex <==
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{eqnarray}}
\newcommand{\ea}{\end{eqnarray}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% NUMBERING Chapters, eqs., etc.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}
\numberwithin{table}{section}
\numberwithin{figure}{section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% THEOREM environment
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Defining some environments
\theoremstyle{definition}

  % theorem numbered by: chapter.section.#
  \newtheorem{thm}{Theorem}[section]
  % definition numbered by: chapter.section.#
  \newtheorem{defn}{Definition}[section]
  % proposition, for numbering it is considered
  % as thm-environment
  \newtheorem{prop}[thm]{Proposition}
  % lemma
  \newtheorem{lem}{Lemma}[section]


==> preamble/layout2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% MARGINS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% note: do not use vmargin package in conjunction w/ crop package
% not compactible.



% size of paper
\geometry{papersize={170mm,240mm}}

% set margins of body

%hmargin={leftm,rightm}
\geometry{hmargin={22mm,22mm}}
% vmargin={topm,bottomm}
\geometry{vmargin={16mm,16mm}}
\geometry{voffset=23mm,hoffset=20mm}
% set position and height of header and footer

% sets size of header
\geometry{headheight={5mm}}
% sets distance between baseline of header and main text
\geometry{headsep={8mm}}
% sets distance between baseline of last line of text and baseline of footer
\geometry{footskip={12mm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% HEADERS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% to get nice headers

% turn on fancy headers
\pagestyle{fancyplain}

\renewcommand{\chaptermark}[1]%
              {\markboth{#1}{}}
\renewcommand{\sectionmark}[1]%
              {\markright{\thesection\ #1}}

\lhead[\fancyplain{}{\bf \thepage}]%
       {\fancyplain{}{\nouppercase{\bf \rightmark}}}
\rhead[\fancyplain{}{\nouppercase{\bf \leftmark}}]%
       {\fancyplain{}{\bf \thepage}}
\cfoot{}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TABLES AND FIGURES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\captionsetup{labelsep=period,labelfont={small,bf},textfont=small}

